On the Exploration of LM-Based Soft Modular Robot Design

Recent large language models (LLMs) have demonstrated promising capabilities in modeling real-world knowledge and enhancing knowledge-based generation tasks. In this paper, we further explore the potential of using LLMs to aid in the design of soft modular robots, taking into account both user instructions and physical laws, to reduce the reliance on extensive trial-and-error experiments typically needed to achieve robot designs that meet specific structural or task requirements. Specifically, we formulate the robot design process as a sequence generation task and find that LLMs are able to capture key requirements expressed in natural language and reflect them in the construction sequences of robots. To simplify, rather than conducting real-world experiments to assess design quality, we utilize a simulation tool to provide feedback to the generative model, allowing for iterative improvements without requiring extensive human annotations. Furthermore, we introduce five evaluation metrics to assess the quality of robot designs from multiple angles including task completion and adherence to instructions, supporting an automatic evaluation process. Our model performs well in evaluations for designing soft modular robots with uni- and bi-directional locomotion and stair-descending capabilities, highlighting the potential of using natural language and LLMs for robot design. However, we also observe certain limitations that suggest areas for further improvement.

==> sections/validations.tex <==
\section{Explaining the Trained Models}
The capability of the proposed model to design proper robots given three different goals has been proven in Section \ref{sct:experiments}, while the way in which the model functions remains in the dark.
This section presents additional explanatory experiments to examine whether the model generates working robot structures purely out of luck or based on its understanding of the instructions (i.e., the task objective, the environment, and necessary components for accomplishing the task).
Specifically, we set up 5 tasks that require geometric knowledge about the environment or the functionality of sub-robot components to the target tasks and examined whether such knowledge is encoded by the three models trained for the three task objectives in our experiments.
All the weights of the models we trained are frozen in these experiments and a prediction head is trained on top of the model weights for each task.
Section \ref{sct:validation-task:introduction} formally defines these tasks and introduces the evaluation metric of each task, and the validation results are presented in Sections \ref{sct:validation-task:task-1} - \ref{sct:validation-task:task-5}.

\subsection{Explanatory Tasks and Evaluation Schemes} \label{sct:validation-task:introduction}
The 5 explanatory tasks involve (1) space filling, (2) path finding, (3)

